Reasoning Abilities of Large Language Models: In-Depth Analysis on the Abstraction and Reasoning Corpus

The existing methods for evaluating the inference abilities of Large Language Models (LLMs) have been predominantly results-centric, making it challenging to assess the inference process comprehensively. We introduce a novel approach using the Abstraction and Reasoning Corpus (ARC) benchmark to evaluate the inference and contextual understanding abilities of LLMs in a process-centric manner, focusing on three key components from the Language of Thought Hypothesis (LoTH): Logical Coherence, Compositionality, and Productivity. Our carefully designed experiments reveal that while LLMs demonstrate some inference capabilities, they still significantly lag behind human-level reasoning in these three aspects. The main contribution of this paper lies in introducing the LoTH perspective, which provides a method for evaluating the reasoning process that conventional results-oriented approaches fail to capture, thereby offering new insights into the development of human-level reasoning in artificial intelligence systems.

==> contents/6.6_human_analysis_tool.tex <==
\subsection{Compositionality Analysis on Human Performance}

To establish a comparison baseline for LLMs' compositionality, we conducted human performance measurements under identical experimental constraints. We developed a specialized tool (Fig.~\ref{figures/Appendix/Tool}) that provides the same information available to LLMs: ARC task demonstration examples, initial test input, current grid state, DSL functions, and object information extracted through PnP.

The tool enables single-pixel selection through grid clicks and object selection via dedicated buttons. Invalid parameter combinations result in step incrementation without execution. For example, DSL \textit{Horizontal Line} requires two pixels with identical y-values; mismatched pixel coordinates trigger step incrementation without execution.

\begin{figure}[ht]
   \centering
   \includegraphics[width=\columnwidth]{figures/6_Appendix/Tool.pdf}
   \caption{Performance measurement tool for human participants: The interface consists of five numbered sections: 1) Sample input-output pairs from the given ARC task; 2) Test input grid for the given task; 3) Current grid for participants' responses; 4) Available DSLs; and 5) Object information automatically extracted using the PnP method. Participants must utilize the provided DSLs and object information to construct appropriate solutions, with both grid pixels and objects available as function parameters. Participants are meant to click complete if the current grid seems to be the solution.}
   \label{figures/Appendix/Tool}
\end{figure}

We conducted experiments with seven participants across 260 ARC tasks, maintaining the same constraints as LLMs: a 10-step solution limit and exclusive use of provided DSLs. Tasks requiring grid size changes were excluded. Performance was evaluated based on exact matches between final and target outputs (scored as 1 for correct and 0 for incorrect).

Key findings are as follows:
\begin{itemize}
   \item Of 260 tasks, 158 were solvable within the given constraints (10 steps, provided DSLs)
   \item Participants solved an average of 137 tasks, achieving approximately 86\% accuracy on solvable tasks
\end{itemize}

These findings served as a baseline for our comparative analysis of LLMs' compositionality.

==> contents/Compositionality_tool.tex <==
LLMs의 Compositionality의 비교 대상으로 인간의 성능을 측정하고자 하였다. LLMs과 동일한 실험 셋팅에서 인간의 Compositionality을 평가해야 하기 때문에 동일한 제약 조건 아래에서 실험이 이뤄져야 한다. 이를 위해 Fig. ~\ref{figures/Appendix/Tool}와 같은 tool을 만들어 실험에 사용했다. 해당 tool은 LLMs에게 제공했던 정보인 ARC task의 demonstration examples와 초기 test input와 현재 grid 상태, 각 DSL 함수들, PnP를 통해 추출한 object 정보들이 주어진다. DSL 함수들은 함수 종류에 따라 전체 그리드, 픽셀, obejct 등의 여러 인자를 사용한다. DSL 종류는 크게 color change, transformation, complete 등으로 나눠지며 어떤 인자의 종류를 받는지에 따라 세부적인 DSL 함수들이 구분되어 진다. 좌표를 인자로 받는 color change 함수에는 좌표와 object 만을 인자로 받으며 좌표를 인자로 받는 경우는 Pixel Color, X Line, Horizontal Line, Vertical Line, Diagonal Line 등이 있다. 해당 함수를 사용하는 방법은 Fig.~\ref{figures/Appendix/Tool}의 test input grid에서 타켓이 되는 좌표와 색상을 선택하고 사용하고자 하는 DSL을 선택하면 된다. 이때 Horizontal Line, Vertical Line, Diagonal Line 등은 2개의 좌표를 받는데 이때 shift키를 누르고 선택하면 2개의 좌표가 선택된다. 만약, 사용할 함수에 적절하지 않는 인자들어가게 될 경우, 함수가 실행되지 않고 step을 1 증가시킨다. 예를 들어, Horizontal Line의 경우, 인자로 받는 2개의 좌표가 서로 수평하게 있지 않은 경우, 즉 2개의 좌표의 y의 값이 다른 경우, Horizontal Line을 수행하지 않게 된다. Coloar change 중 object를 인자로 받는 DSL은 Object Color 가 있으며 Fig.~\ref{figures/Appendix/Tool}의 오른쪽에 있는 object를 클릭한 후 변경하고자 하는 색상 및 Object Color DSL을 선택하면 된다. Transformation에 대한 DSLs은 Object를 인자로 받거나 전체 grid를 인자로 받는 경우가 있다. Object를 인자로 받는 경우, object 정보 중 하나를 클릭한 후, Rotate Left Obj, Roate Right Obj, Horizontal Flip Obj, Vertical Flip Obj, Move Left, Move Right, Move Up, Move Down 등의 DSLs 중 하나를 선택하면 된다. Transformation 중 전체 Grid를 인자로 받는 경우에는 인자를 선택할 필요없이 Rotate Left, Rotate Right, Horizontal Flip, Verical Flip 등의 DSLs 중 하나를 선택하며 전체 grid가 해당 dsl에 맞게 transformation을 수행한다.

\begin{figure}[ht]
    \centering
    \includegraphics[width=\columnwidth]{figures/Appendix/Tool.pdf}
    \caption{인간 성능을 측정하기 위해 사용된 Tool: Tool의 왼쪽에는 task의 demonstration examples가 있으며 중앙에는 test input과 현재 그리드의 상태, DSLs들이 제공된다. 현재 그리드 상태에서 픽셀을 클리하면 해당 픽셀을 인자로 사용할 수 있다. 오른쪽에는 test input에서 PnP를 통해 추출한 objects 정보들이 있으며 주황색 버튼을 클릭하면 해당 object를 인자로 사용할 수 있다.}
    % \caption{Accuracy and number of tasks per step in the DSL understanding experiment. This experiment was repeated 10 times for 158 tasks. The blue bars represent the accuracy for each step, and the red line shows the number of trials for each step. As the number of steps increases, accuracy tends to decrease.}\label{fig:Main_Experiments/understanding_dsl_graph}
    \label{figures/Appendix/Tool}
\end{figure}
인간은 주어진 정보들을 활용하여 적절한 test output을 만들도록 현재 grid에서 어떤 DSL과 인자들을 사용하여 test input의 상태를 바꿀지를 결정해야 한다. 이때 LLMs과 동일하게 10 step 안에 task를 해결해야 하며 DSL을 잘못 사용하는 경우에는 test input의 상태는 바뀌지 않고 step만 증가하게 된다. 또한, 제공된 DSL만을 가지고 풀 수 있어야 하기 때문에 test input과 올바른 test output의 grid size가 다른 tasks들은 베재하였다. 이렇게 해서 ARC training과 evaluation dataset 중 총 260개의 tasks에 대해서 10 step 안에 인간이 문제를 풀어보도록 한 실험을 진행하였으며 task id, 사용한 dsl 및 인자, 소요된 step 등의 정보를 수집하였다.

총 7명의 참가자를 통해 260개의 tasks에 대해서 인간 성능을 측정하였으며 이때 최종 test input의 grid가 정답과 일치하는지를 확인하였고 일치했을때는 1, 틀렸다면 0을로 체크하여 평균을 구하였다. 또한, 모든 참가자가 풀지 못한 문제에 대해서 여러 번의 검토를 통해 해당 문제가 주어진 DSL을 가지고 10 step 이내에 풀 수 있는지를 확인해 보았다. 

주어진 DSLs과 object 정보 등을 이용해서 10 step 이내에 풀 수 있는 문제들은 260문제 중 158문제 였으며 이에 대해서 평균적으로 137문제를 풀었으며 이는 풀 수 있는 문제 158개에 대한 평균 정확도가 약 86\%정도임을 뜻한다.  
인간 실험을 통해 알아낸 점은 크게 2가지 이다. 하나는 주어진 DSL 및 여러 제약 조건 아래에서 풀 수 있는 ARC 문제 158개를 선별했다는 것이며 다른 하나는 158개의 task에 대한 인간의 계획 능력을 평가했다는 점이다. 이러한 결과는 LLMs의 Compositionality을 평가하는 실험 및 결과를 분석하는 과정에 사용되었다. 
